Compositional Physical Reasoning of Objects and Events from Videos

Understanding and reasoning about objects' physical properties in the natural world is a fundamental challenge in artificial intelligence. While some properties like colors and shapes can be directly observed, others, such as mass and electric charge, are hidden from the objects' visual appearance. This paper addresses the unique challenge of inferring these hidden physical properties from objects' motion and interactions and predicting corresponding dynamics based on the inferred physical properties. We first introduce the Compositional Physical Reasoning (ComPhy) dataset. For a given set of objects, ComPhy includes limited videos of them moving and interacting under different initial conditions. The model is evaluated based on its capability to unravel the compositional hidden properties, such as mass and charge, and use this knowledge to answer a set of questions. Besides the synthetic videos from simulators, we also collect a real-world dataset to show further test physical reasoning abilities of different models. We evaluate state-of-the-art video reasoning models on ComPhy and reveal their limited ability to capture these hidden properties, which leads to inferior performance. We also propose a novel neuro-symbolic framework, Physical Concept Reasoner (PCR), that learns and reasons about both visible and hidden physical properties from question answering. After training, PCR demonstrates remarkable capabilities. It can detect and associate objects across frames, ground visible and hidden physical properties, make future and counterfactual predictions, and utilize these extracted representations to answer challenging questions.

==> figures/rebuttal/new_cap1.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/rebuttal/new_cap_1_v3.pdf}
    \vspace{-1em}
    \caption{An example of combining the strength of \modelNew and LVLMs to enable new commonsense reasoning capabilities. The LVLM is able to write a program in Python (Figure~\ref{fig:code1}) that calls the reasoning modules (\texttt{get\_color} and \texttt{filter\_out}) in \modelNew and (\texttt{llm\_query}) from LVLMs to handle the problem and provides the correct answer with explanation.}
    \label{fig:newcap}
 \begin{minipage}[t]{1\linewidth}
        %\centering
        \begin{minted}[
        frame=lines,
        framesep=2mm,
        fontsize=\footnotesize,
        bgcolor=Gray,
        numbersep=5pt,
        escapeinside=||,
        linenos
        ]{python}
def execute_command(video, possible_answers, query, ImagePatch,
            VideoSegment, llm_query, bool_to_yesno, distance, best_image_match):
    video_segment = VideoSegment(video)
    num_objects = video_segment.count_objects()
    # Find the first object that gets out of the scene
    out_list = []
    for idx in range(num_objects):
        out_frm = video_segment.filter_out(idx)
        if out_frm is not None:
            out_list.append([idx, out_frm])
    if len(out_list) == 0:
        return "There is no object that exits the scene"
    out_list = sorted(out_list, key=lambda x: x[1])
    first_out_idx = out_list[0][0]
    # Find the gray object
    gray_obj_idx = None
    for idx in range(num_objects):
        color = video_segment.get_color(idx)
        if color == 'gray':
            gray_obj_idx = idx
            break
    if gray_obj_idx is None:
        return "There is no gray object in the video"
    # Get shapes of the gray object and the first object that gets out
    gray_shape = video_segment.get_shape(gray_obj_idx)
    first_out_shape = video_segment.get_shape(first_out_idx)
    # Use llm_query to determine stability
    answer = llm_query(f"Will it be stable to stack a {gray_shape} on 
                a {first_out_shape}?")
    return answer
     \end{minted}
    \centering
\end{minipage}
     \caption{The program that the LVLM generates to handle the query in Figure~\ref{fig:newcap}. The program first calls the modules (\texttt{get\_color} and \texttt{filter\_out}) in \modelNew to identify the object 4 and the object 2 in the video. The program that calls the \texttt{get\_shape} module in \modelNew to get the objects' shape and finally sends the LVLM a question based on the shape to identify the stability of the structure and gives the explanation (the \textbf{\red{answer}} in Figure~\ref{fig:newcap}).}
    \label{fig:code1}
\end{figure*}

==> figures/rebuttal/new_cap1_v2.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/rebuttal/new_cap_1_v2.pdf}
    \vspace{-1em}
    \caption{An example of combining the strength of \modelNew and LVLMs to enable new commonsense reasoning capabilities. The LVLM is able to write a program in Python (Figure~\ref{fig:code1}) that calls the reasoning modules (\texttt{get\_color} and \texttt{get\_mass}) in \modelNew and (\texttt{llm\_query}) from LVLMs to handle the problem and provides the correct answer with explanation.}
    \label{fig:newcap}
 \begin{minipage}[t]{1\linewidth}
        %\centering
        \begin{minted}[
        frame=lines,
        framesep=2mm,
        fontsize=\footnotesize,
        bgcolor=Gray,
        numbersep=5pt,
        escapeinside=||,
        linenos
        ]{python}
def execute_command(video, possible_answers, query, ImagePatch, 
        VideoSegment, llm_query, bool_to_yesno, distance, best_image_match):
    video_segment = VideoSegment(video)
    num_objects = video_segment.count_objects()
    heavy_obj_idx = None
    gray_obj_idx = None
    for idx in range(num_objects):
        mass_label = video_segment.get_mass(idx)
        color = video_segment.get_color(idx)
        shape = video_segment.get_shape(idx)
        if mass_label == 'heavy':
            heavy_obj_idx = idx
        if color == 'gray':
            gray_obj_idx = idx
    if heavy_obj_idx is None or gray_obj_idx is None:
        return 'Cannot find the described objects!'
    heavy_shape = video_segment.get_shape(heavy_obj_idx)
    gray_shape = video_segment.get_shape(gray_obj_idx)
    answer = llm_query(f'Will it be stable to stack a {gray_shape} 
        on a {heavy_shape}?')
    return answer
     \end{minted}
    \centering
\end{minipage}
     \caption{The program that the LVLM generates to handle the query in Figure~\ref{fig:newcap}. The program first calls the modules () in \modelNew to identify
    \label{fig:code1}
    }
\end{figure}

==> figures/rebuttal/new_cap_v2.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/rebuttal/new_cap_v2_2_ori.pdf}
    \vspace{-1em}
    \caption{An input video and a language instruction to ask AI models to edit the target video.}
    \label{fig:video1}
 \begin{minipage}[t]{1\linewidth}
        %\centering
        \begin{minted}[
        frame=lines,
        framesep=2mm,
        fontsize=\footnotesize,
        bgcolor=Gray,
        numbersep=5pt,
        escapeinside=||,
        linenos
        ]{python}
def execute_command(video) -> list:
    video_segment = VideoSegment(video)
    num_objects = video_segment.count_objects()
    red_obj_idx = None
    for idx in range(num_objects):
        color = video_segment.get_color(idx)
        if color == 'red':
            red_obj_idx = idx
            break
    if red_obj_idx is not None:
        edited_images = video_segment.edit_objects(red_obj_idx, "golf ball")
        return edited_images
    return []
     \end{minted}
    \centering
\end{minipage}
    \vspace{-1em}
    \caption{Program generated by the LVLM to address the query in Figure~\ref{fig:video1}. It first uses the \texttt{get\_color} module to locate the red object, then applies the Stable Diffusion–based \texttt{edit\_objects} module to transform that region into a \textit{golf ball}. Integrating \modelNew with LVLMs empowers the model to incorporate new modules for new tasks such as video editing.
    \label{fig:code2}
    }
    \centering
    \includegraphics[width=\textwidth]{figures/rebuttal/new_cap_v2_2_edit.pdf}
    \vspace{-1em}
    \caption{The output video of replacing the \red{red} object with a \textbf{golf ball} by calling the new stable diffusion module (\texttt{edit\_object})~\cite{Rombach_2022_CVPR} to edit the target object region.}
    \label{fig:video2}
\end{figure*}

==> rebuttal/tab_cmp.tex <==
\begin{table*}[ht]
    \centering
    \begin{tabular}{lcccc}
        \toprule
         &  Shape Categories & Background Scenes & Colors & Answer Space \\
        \midrule
        \dataset &3 &1 &8 &88\\
        \datasetNew &13 &9 &8 &175 \\
        \bottomrule
    \end{tabular}
    \caption{Comparison of the original \dataset and the new \datasetNew.~\zf{to fill}}
    \label{tab:cmp}
\end{table*}

==> rebuttal/tab_cmp_revise.tex <==
\begin{table*}[ht]
    \centering
    \begin{tabular}{lcccc}
        \toprule
         &  Shape Categories & Background Scenes & Colors & Answer Space \\
        \midrule
        \dataset &3 &1 &8 &88\\
        \datasetNew &13 &9 &8 &175 \\
        \bottomrule
    \end{tabular}
    \caption{\revise{Comparison of the original \dataset and the new \datasetNew.~\zf{to fill}}}
    \label{tab:cmp}
\end{table*}

==> rebuttal/tab_parsing.tex <==
\begin{table*}[t]
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{ll}
    \toprule
    Question & What would be the outcome if the sphere had a greater \blue{mass}? \\
    \midrule
    PCR’s parser
      & all\_events, objects, sphere, filter\_shape, unique, \red{counterfact\_uncharged}, filter\_counterfact, belong\_to, \red{not} \\
    LVLMs
        & all\_events, objects, sphere, filter\_shape, unique, counterfact\_heavier, filter\_counterfact, belong\_to \\
    \midrule
    Question & What color is the metal sphere that remains stationary at the \blue{start} of the video? \\
    \midrule
    PCR’s parser
          & objects, metal, filter\_material, sphere, filter\_shape, \red{filter\_end}, query\_frame, filter\_stationary, query\_color \\
    LVLMs
          & objects, metal, filter\_material, sphere, filter\_shape, \red{filter\_start}, query\_frame, filter\_stationary, query\_color \\
    \bottomrule
  \end{tabular}
   }
  \caption{Comparison of parsing results between \modelNew’s program parser and LVLMs. \modelNew’s parser fails on the revised questions due to distribution shift from its original training set, whereas LVLMs succeed thanks to superior generalization. Key operators are highlighted in \red{red}.}
  \label{tab:parse}
\end{table*}




==> rebuttal/tab_question.tex <==
\begin{comment}
\begin{table}[t]
    \centering
    \begin{tabular}{l|l}
        \toprule
        Original Question 1 
          & If the cyan sphere were heavier, what would not happen?  \\
        \midrule
        \multirow[c]{4}{*}{\multicolumn{1}{c}{Revised Question 1}} 
          & What would not occur if the cyan sphere had more weight?     \\
          & If the cyan sphere had more mass, what outcome would be impossible? \\
          & What would not occur if the cyan sphere were to have a greater weight? \\
          & What would not occur if the cyan sphere had more weight?      \\
        \midrule
        Original Question 2 
          & What will happen next?                                      \\
        \midrule
        \multirow[c]{4}{*}{\multicolumn{1}{c}{Revised Question 2}} 
          & What is the next event that will take place?               \\
          & What is likely to happen next?                             \\
          & What is the next event that will occur?                    \\
          & What is expected to happen next?                           \\
        \bottomrule
    \end{tabular}
    \caption{Sampled revised questions of the same semantics as the original questions. The revised questions have the same semantics as the original questions but have more diverse and flexible language description, which pose challenges for language parsers~\cite{yi2019clevrer,chen2021grounding} that have not seen these textual distribution during training.}
    \label{tab:revise}
\end{table}
\end{comment}

\begin{table*}[t]
  \centering
  \begin{tabular}{c|l}
    \toprule
    Original Question 1 
      & If the cyan sphere were heavier, what would not happen? \\
    \midrule
    \multirow{4}{*}{Revised Question 1} 
      & What would not occur if the cyan sphere had more weight?     \\
      & If the cyan sphere had more mass, what outcome would be impossible? \\
      & What would not occur if the cyan sphere were to have a greater weight? \\
      & What would not occur if the cyan sphere had more weight?      \\
    \midrule
    Original Question 2 
      & What will happen next?                                      \\
    \midrule
    \multirow{4}{*}{Revised Question 2} 
      & What is the next event that will take place?               \\
      & What is likely to happen next?                             \\
      & What is the next event that will occur?                    \\
      & What is expected to happen next?                           \\
    \bottomrule
  \end{tabular}
  \caption{{Examples of revised questions that preserve the original semantics while exhibiting greater linguistic diversity and flexibility. These variations challenge language parsers~\cite{yi2019clevrer,chen2021grounding} by introducing textual patterns not encountered during training.}}
  \label{tab:revise}
\end{table*}




==> table_revise/tab_diverse.tex <==
\begin{table*}[t]
\begin{center}
%\small
\setlength{\tabcolsep}{8pt}
\begin{tabular}{llccccc}
\toprule
\multirow{2}{*}{Categories} & \multirow{2}{*}{Methods}  & \multirow{2}{*}{Factual} & \multicolumn{2}{c}{Predictive} &  \multicolumn{2}{c}{Counterfactual} \\
%\cmidrule(lr){5-6}\cmidrule(lr){7-8}
  &             &               & per opt.       & per ques.      & per opt.      & per ques.     \\
\midrule
\multirow{3}{*}{Bias analysis models} 
& Random    &1.8 &50.1 &22.9 &48.1 &24.0      \\
& Frequent  &15.7 &50.0 &0.0 &50.0 &0.0          \\
& Blind-LSTM    &43.2  &50.3  &25.0  &49.2  &23.2            \\

\midrule
\multirow{2}{*}{video question answering  models} 
& CNN-LSTM~\cite{antol2015vqa}    &49.6  &52.8  &29.9  &55.7  &29.7             \\
& HCRN~\cite{le2020hierarchical}  &51.5  &\Scnd{56.3}  & \Scnd{34.1}  &51.9  &30.1             \\
\midrule
\multirow{2}{*}{Compositional reasoning
models} 
& MAC~\cite{hudson2018compositional}     & \Scnd{51.7}  &50.4  &28.9  &51.9  &26.3      \\
& ALOE~\cite{ding2020object}         &46.9  &52.4  &29.0  &51.5  &28.6              \\
\midrule
\multirow{3}{*}{Models with Reference Videos}
& {CNN-LSTM (Ref)}~\cite{antol2015vqa}      &49.7  &51.4  &23.3  &55.6  &30.5      \\
& {MAC (Ref)}~\cite{hudson2018compositional}    &50.6  &51.9  &33.3  &50.8  &25.2  \\
& ALOE (Ref)~\cite{ding2020object}      &48.6  &51.2  &26.1  &52.9  &27.2       \\
\midrule

\multirow{4}{*}{Large Vision Language Models} 
& ALPRO~\cite{li2022align}  &47.1  &51.8  &28.9  &52.6  &28.4   \\
& GPT-4o-mini~\cite{achiam2023gpt} &42.5  &50.0  &29.2  & \Scnd{58.8}  & \Scnd{30.7}       \\
& Gemini~\cite{team2023gemini} &34.2  &50.3  &25.7  &49.4  &30.6     \\
\midrule
& \textbf{PCR(ours)}  & \Frst{68.4}  & \Frst{58.3}  & \Frst{34.9}  & \Frst{60.3}  & \Frst{32.8}        \\
\midrule
& {Human Performance}  &88.6  &82.9  &73.7  &88.2  &78.9      \\
\bottomrule
\end{tabular}
\end{center}
\vspace{-1em}
\caption{{Evaluation of physical reasoning on \datasetNew. {Human performance is based on sampled questions. See the text for more details. \Frst{Red} text and \Scnd{blue} text indicate the first and the second best results other than human performance.}}}
%\zf{Need more baselines.}} 
% \sld{modify color}
\label{tab:diverse}
\end{table*}

==> table_revise/tab_prog.tex <==
\begin{table*}[thbp]
    \centering
    %\caption{Performance Analysis of \modelNew and PCR+LVLMs. \modelNew’s parser fails on the revised questions due to distribution shift from its original training set, whereas LVLMs succeed thanks to superior generalization.}
    \begin{tabular}{lcccccc}
        \toprule
         \multirow{2}{*}{Methods}  & \multirow{2}{*}{Factual} & \multicolumn{2}{c}{Predictive} &  \multicolumn{2}{c}{Counterfactual} \\
          &               & per opt.       & per ques.      & per opt.      & per ques.     \\
        \midrule
        \modelNew & 51.9 & 60.6 & 44.2 & 57.4 & 41.5  \\
        PCR+LVLMs & 69.7 & 73.5 & 54.0 & 76.3 & 60.9  \\
        \bottomrule
    \end{tabular}
    \caption{Performance Comparison of \modelNew and PCR+LVLMs on revised questions, where \modelNew fails under a distribution shift from its training set, whereas PCR+LVLMs succeed thanks to superior generalization.}
    \label{tab:metrics_transposed}
\end{table*}


==> table_revise/tab_real.tex <==
\begin{table*}[t]
\begin{center}
%\small
\setlength{\tabcolsep}{8pt}
\begin{tabular}{llccccc}
\toprule
\multirow{2}{*}{Categories} & \multirow{2}{*}{Methods}  & \multirow{2}{*}{Factual} & \multicolumn{2}{c}{Predictive} &  \multicolumn{2}{c}{Counterfactual} \\
  &             &               & per opt.       & per ques.      & per opt.      & per ques.     \\
\midrule
\multirow{3}{*}{Bias analysis models} 
& Random      &7.6 &50.0 &25.0 &50.9 &20.8                 \\
& Frequent    &41.7 &53.6 &28.7 &50.0 &23.9                                  \\
& Blind-LSTM    &50.6  &61.5 &46.0 &51.9 &32.2            \\

\midrule
\multirow{2}{*}{video question answering  models} 
& CNN-LSTM~\cite{antol2015vqa}    &55.6  &64.2 &47.3 &50.9 &33.3           \\
& HCRN~\cite{le2020hierarchical}  &51.9  &62.5 &53.5 &50.9 &32.1               \\
\midrule
\multirow{2}{*}{Compositional reasoning
models} 
& MAC~\cite{hudson2018compositional}      &58.9  &60.9 & \Scnd{57.1} & \Scnd{52.8} & \Scnd{35.8}        \\
& ALOE~\cite{ding2020object}         &60.8  &60.6 &42.4 &47.1 &28.7             \\
\midrule
\multirow{3}{*}{Models with Reference Videos}
& {CNN-LSTM (Ref)}~\cite{antol2015vqa}      &49.0  & \Scnd{64.3} &41.3 &50.0 &26.3           \\
& {MAC (Ref)}~\cite{hudson2018compositional}    &56.4  &56.2 &46.4 &51.4 &34.9         \\
& ALOE (Ref)~\cite{ding2020object}      & \Scnd{61.6}  &61.4 &42.8 &51.6 &32.1          \\
\midrule

\multirow{4}{*}{Large Vision Language Models} 
& ALPRO~\cite{li2022align}  &50.9  &55.3 &39.2 &49.7 &29.2  \\
& GPT-4o-mini~\cite{achiam2023gpt} &42.6  &49.6 &23.2 &47.5 &26.0        \\
& Gemini~\cite{team2023gemini} &32.5  &57.7 &23.1 &52.1 &29.8   \\
\midrule
& \textbf{PCR(ours)}  & \Frst{63.5}  &\Frst{70.4} & \Frst{62.7} & \Frst{54.6} & \Frst{36.5}      \\
& {Human Performance}   &90.0  &95.0 &90.0 &94.4 &88.9     \\
\bottomrule
\end{tabular}
\end{center}
\vspace{-1em}
\caption{Evaluation of physical reasoning on \datasetNewReal. {Human performance is based on sampled questions. See the text for more details. \Frst{Red} text and \Scnd{blue} text indicate the first and the second best results other than human performance.}}
\label{tb:real}
\end{table*}

==> table_revise/tab_real_ori.tex <==
\begin{table*}[t]
\begin{center}
%\small
\setlength{\tabcolsep}{8pt}
\begin{tabular}{llccccc}
\toprule
\multirow{2}{*}{Categories} & \multirow{2}{*}{Methods}  & \multirow{2}{*}{Factual} & \multicolumn{2}{c}{Predictive} &  \multicolumn{2}{c}{Counterfactual} \\
%\cmidrule(lr){5-6}\cmidrule(lr){7-8}
  &             &               & per opt.       & per ques.      & per opt.      & per ques.     \\
\midrule
\multirow{3}{*}{Models with Reference Videos}
& {CNN-LSTM (Ref)}~\cite{antol2015vqa}                \\
& {MAC (Ref)}~\cite{hudson2018compositional}            \\
& ALOE (Ref)~\cite{ding2020object}               \\
\midrule
\multirow{4}{*}{Large Vision Language Models} & 
ALPRO~\cite{li2022align}  & \\
& GPT-4V~\cite{achiam2023gpt} &       \\
& Gemini~\cite{team2023gemini} &   \\
\midrule

& {Human Performance}        \\
\bottomrule
\end{tabular}
\end{center}
\caption{Evaluation of ALOE and human performance on physical reasoning on \datasetNewReal.}
%\zf{Need more baselines.}} 
% \sld{modify color}
\label{tb:real_ori}
\end{table*}

==> tables/tab_abs.tex <==
\begin{table*}[t]
    \centering
    \setlength{\tabcolsep}{8pt}
    \begin{tabular}{lcccccccc}
    \toprule
    \multirow{2}{*}{Methods} & \multirow{2}{*}{Property Labels} & \multirow{2}{*}{Factual} & \multicolumn{2}{c}{Predictive} &  \multicolumn{2}{c}{Counterfactual} \\
    \cmidrule(lr){4-5}\cmidrule(lr){6-7}
     &         &      & per opt.       & per ques.      & per opt.      & per ques. &         \\   
    \midrule
    \revise{\modelNew w/o R} & - &  68.7   &   52.0         &  28.1 &    54.9        &  28.0       \\
    \revise{\modelNew w/o CI} & -  &  70.3    &    51.2        &  24.4      &   54.0         &  28.0  \\
    %\revise{\modelNew with GT-D} & - &  78.0    &    79.5        &  59.8      &   76.3         &  53.6  \\
    %\revise{\modelNew+GT-PL.} & \checkmark *  &  73.6    &    77.0        &  59.5      &   72.3         &  52.9  \\
    \revise{{\modelNew}}  & - &  78.3        &  75.0        &  56.5   &     70.5       &  50.2     \\
    \bottomrule
    \end{tabular}
    \caption{Ablation study of \modelNew on \dataset. $\checkmark$ denotes the models uses dense property labels for training. $\checkmark *$ denotes the ablation models that using the ground-truth property labels for dynamic prediction. Best performance is in bold face. \label{tb:abs}}
\end{table*}

==> tables/tab_baseline.tex <==
\begin{table*}[t]
\begin{center}
%\small
\setlength{\tabcolsep}{8pt}
\begin{tabular}{llccccc}
\toprule
\multirow{2}{*}{Categories} & \multirow{2}{*}{Methods}  & \multirow{2}{*}{Factual} & \multicolumn{2}{c}{Predictive} &  \multicolumn{2}{c}{Counterfactual} \\
%\cmidrule(lr){5-6}\cmidrule(lr){7-8}
  &             &               & per opt.       & per ques.      & per opt.      & per ques.     \\
\midrule
\multirow{3}{*}{Bias analysis models} & Random                   &  29.7         & 51.9      & 22.6               &    49.7           &    9.1                      \\
& Frequent                 &  30.9         &  56.2     &  25.7 &    50.3       &  8.7                         \\
& Blind-LSTM               & 39.0          & 57.9          & 28.7      &  55.7           &    12.5  \\

\midrule
\multirow{2}{*}{video question answering  models} & CNN-LSTM~\cite{antol2015vqa}                 & 46.6          & 59.5          &  29.8        & 58.6               &  14.6     \\
& HCRN~\cite{le2020hierarchical}                     & 47.3          &  62.7         &   32.7       & 58.6               &  14.2   \\
\midrule
\multirow{2}{*}{Compositional reasoning
models} & MAC~\cite{hudson2018compositional}                      &   \Frst{68.6}        & 60.2      &  32.2    &    60.2           &    16.0   \\
%mac (ref)                &   -           &          &          &           &       \\
& ALOE~\cite{ding2020object}                     &   54.3        &   \Scnd{65.9}    &    35.2  &     \Scnd{65.4}  & \Scnd{20.8}      \\
%\revise{SlotFormer (Ref)} \\
\midrule
\multirow{3}{*}{Models with Reference Videos}
& {CNN-LSTM (Ref)}~\cite{antol2015vqa}                &  {41.9}   &      {59.6}     &  {29.4}  &  {57.2}     &      {12.8}  \\
& {MAC (Ref)}~\cite{hudson2018compositional}                      &   
\Scnd{65.8}        &      {60.2}     &  {30.7}     &   {60.3}           &      {14.3} \\
& ALOE (Ref)~\cite{ding2020object}               &   57.7        &  \Frst{67.9}     &  \Scnd{37.1}        &  \Frst{67.9}   &   \Frst{22.2}   \\
\midrule

\multirow{4}{*}{Large Vision Language Models} & 
ALPRO~\cite{li2022align}  & {45.2}        &      {56.9}     &  {27.2}     &   {53.7}           &      {14.4} \\
& GPT-4V~\cite{achiam2023gpt} &   {42.2}             &   {60.7}           &      \Frst{47.1}  &      {51.1}     &  {8.9} \\
& Gemini~\cite{team2023gemini} &   {37.7}             &   {46.5}           &      {22.7}  &      {49.2}     &  {6.3} \\
\midrule

& {Human Performance}               &   {90.6}        &  {88.0}     &  {75.9}        &  {80.0}      &   {52.9}   \\
\bottomrule
\end{tabular}
\end{center}
\vspace{-1em}
\caption{Evaluation of physical reasoning on \dataset. {Human performance is based on sampled questions. See Section~\ref{sec:eval} for more details. \Frst{Red} text and \Scnd{blue} text indicate the first and the second best results other than human performance.}}
%\vspace{-1em}
%\zf{Need more baselines.}} 
% \sld{modify color}
\label{tb:qa}
\end{table*}

==> tables/tab_model.tex <==
\begin{table*}[t]
    \centering
    \setlength{\tabcolsep}{8pt}
    \begin{tabular}{lcccccccc}
    \toprule
    \multirow{2}{*}{Methods} & \multirow{2}{*}{Property Labels} & \multirow{2}{*}{Factual} & \multicolumn{2}{c}{Predictive} &  \multicolumn{2}{c}{Counterfactual} \\
    \cmidrule(lr){4-5}\cmidrule(lr){6-7}
     &         &      & per opt.       & per ques.      & per opt.      & per ques. &         \\
    \midrule
    {NS-DR+}   & \checkmark * &  -           & {73.3}           &  {50.8}   &   {61.1}         & {16.6}      \\
    %{CPL-Gt}   &  \checkmark * & {100}           &  {87.6}    &   {74.0}     & {74.0}         & {35.3}      \\
    \model          &  \checkmark    &   \textbf{80.5}        & 75.3           &  56.4    &   68.3        & \textbf{29.1}       \\

    \revise{{\modelNew}}  & - &  76.0    &    \textbf{80.0}        &  \textbf{62.0}      &   \textbf{70.0}         &  29.0     \\    
    \bottomrule
    \end{tabular}
    \caption{Evaluation of \modelNew on \dataset. $\checkmark$ denotes the models uses dense property labels for training. $\checkmark *$ denotes the ablation models that using the ground-truth property labels for dynamic prediction. Best performance is in bold face. \label{tb:nsdr}}
\end{table*}

==> tables/tab_real.tex <==
\begin{table}[t]
\begin{center}
%\small
\setlength{\tabcolsep}{2pt}
\begin{tabular}{lccccc}

\toprule
 \multirow{2}{*}{Methods}  & \multirow{2}{*}{Factual} & \multicolumn{2}{c}{Predictive} &  \multicolumn{2}{c}{Counterfactual} \\
%\cmidrule(lr){5-6}\cmidrule(lr){7-8}
             &               & per opt.       & per ques.      & per opt.      & per ques.     \\
\midrule
Blind-LSTM  & {51.1}             &   {50.0}           &      {47.4}  &      {53.1}     &  {31.3} \\         
CNN-LSTM~\cite{antol2015vqa}  &   {54.8}             &   {54.2}           &      {47.2}  &      {53.1}     &  {34.4}       \\       
HCRN~\cite{le2020hierarchical}  &    {55.3}             &   \textbf{67.1}           &      {57.9}  &      {46.9}     &  {37.5}      \\        
MAC~\cite{hudson2018compositional}  &   \textbf{61.2}             &   {65.7}           &      {57.0}  &      {53.1}     &  {40.6}     \\         
                  
\midrule
{CNN-LSTM (Ref)}~\cite{antol2015vqa}  &  {53.2}             &   {54.2}           &      {47.2}  &      {51.6}     &  {31.3}        \\   
{MAC (Ref)}~\cite{hudson2018compositional}  &  {59.0}             &   {66.4}           &      \textbf{58.3}  &      {51.6}     &  \textbf{38.7}                 \\
\midrule
ALPRO~\cite{li2022align}  &   {45.3}             &   {48.6}           &      {41.7}  &      {46.8}     &  {32.3}  \\
GPT-4V~\cite{achiam2023gpt} &   {32.0}             &   {44.4}           &      {19.4}  &      \textbf{53.2}     &  {35.4} \\
Gemini~\cite{team2023gemini} &   {5.3}             &   {50.0}           &      {5.2}  &      {48.4}     &  {12.5}\\
%\revise{PCR}&   {65.2}             &   {68.1}           &      {61.1}  &      {56.3}     &  {43.8}\\
\bottomrule
\end{tabular}
\end{center}
\caption{Evaluation of physical reasoning on the real video split of \dataset. The best performance is in boldface.} 
% \zf{remove the performance of our model and analyze it in the later section.}}
\label{tb:real}
\end{table}

==> text/response_to_reviewer1_new_v1.tex <==
%\newpage
\textbf{\red{\section{Response to Reviewer \#1}}}  
\vspace{1em}  
\noindent{\bf \red{Comment 1:} \emph{ComPhy benchmark is too limited and not diverse enough. Its domain is very narrow. The type of objects is constrained to primitive shapes like balls, cubes, or cylinders. The background is always white. The overall setup of the rendered scene is very different from the real world.}}  

\noindent{\bf \red{Response 1:}}  Please refer to the \hyperlink{genresp1}{\red{\textbf{Response to General Concern 1}}}. 

\vspace{1em}\noindent{\bf \red{Comment 2:} \emph{The authors collect a small dataset with real data. However, referring to Figure~4, I found the real data is nearly identical to the simulated data, if not less diverse than it.}}

\noindent{\bf \red{Response 2:}} Please refer to the \hyperlink{genresp2}{\red{\textbf{Response to General Concern 2}}}. 

\vspace{1em}\noindent{\bf \red{Comment 3:} \emph{The authors use magnetism (see page 6 line 17 left column) in real data to simulate "charge" in the rendered data. I'm concerned with whether it will create a discrepancy in behavior of the objects. I'm happy to remove this point from negatives if the authors can provide more details.}} \\
\noindent\textbf{\red{Response 3:}}

Thank you for highlighting this critical point. We use magnetism in our real-world dataset primarily as an analog to simulate electric charges in the rendered data because of their analogous inverse-square law behaviors. While magnetism and electric charges differ fundamentally, their basic interaction dynamics—attraction and repulsion—share substantial mathematical similarities.

Specifically, both electric charges and magnetic dipoles follow analogous inverse-square relationships. Coulomb's law describes the electric force between charges as:

\[ F_{electric} = k_e \frac{q_1 q_2}{r^2}, \]

where \(k_e\) is Coulomb's constant, \(q_1, q_2\) are electric charges, and \(r\) is the distance between charges. Similarly, \textbf{magnetic poles (approximated by dipoles) interact with a force that also depends inversely on the square of the distance between them} (Encyclopædia Britannica, Coulomb’s Law for Magnetism \footnote{\url{https://www.britannica.com/science/magnetism/Repulsion-or-attraction-between-two-magnetic-dipoles?utm_source=chatgpt.com}}), especially under configurations where one pole's interaction dominates, effectively mimicking isolated monopole behavior (
Page 3 of Lehman College Physics Lecture Notes \footnote{\url{https://www.lehman.edu/faculty/dgaranin/Introductory_Physics/PHY167-5-Electromagnetism.pdf}};
Magnetism from Wikipedia~\footnote{\url{https://en.wikipedia.org/wiki/Magnetism}}).

We carefully validated the alignment of these interactions experimentally to minimize any discrepancies between magnetic and charge-based interactions. This ensures the physical reasoning models trained on the real-world magnetic interactions remain applicable and consistent with simulations involving electric charges.

\vspace{1em}\noindent{\bf \red{Comment 4:} \emph{According to Sec 4.1, it seems like some baselines are finetuned on ComPhy while others are unclear. This part will be clearer and stronger if the authors can specify which models are finetuned and why the comparison is fair.}} \\
\noindent{\bf \red{Response 4:} }

Thank you for highlighting this important point. We acknowledge that the original description lacked explicit clarity regarding the fine-tuning of the baselines. Here, we explicitly outline fine-tuning details for each baseline to ensure transparency and fair comparison:

\begin{itemize}[leftmargin=*]
    \item In the family of \textbf{Bias Analysis Models}, \texttt{Random} and \texttt{Frequent} were not fine-tuned, as they intentionally ignore context to reveal statistics biases inherent in \dataset. \texttt{Blind-LSTM} relies on only the textual information of training datasets to study the importance of visual information in the benchmark.
    
    \item \textbf{Visual Question-Answering Models} (\texttt{CNN-LSTM}, \texttt{HCRN}) and \textbf{Visual Reasoning Models} (\texttt{MAC}, \texttt{ALOE}) were all fine-tuned (either trained from scratch or initialized from weights pre-trained on general datasets, such as ImageNet) on the training split of \dataset.

    \item \textbf{Large Vision-Language Models}:
    \begin{itemize}
        \item \texttt{ALPRO} was explicitly fine-tuned on the training split of \dataset, as described.
        \item \texttt{GPT-4V} and \texttt{Gemini} were not fine-tuned due to practical limitations, including model availability and API constraints; hence, their reported performance reflects zero-shot evaluation.
    \end{itemize}
\end{itemize}

 To ensure a fair comparison across different baselines, all fine-tuned models had equal access to the training data, consistent hyperparameter tuning procedures, and evaluation settings. We have integrated this clarification into the revised manuscript for improved transparency and reproducibility. We have revised Sec.~4.1 accordingly and highlight the modification in \revise{red} color in the revised version to describe the details of fine-tuning models and discuss the fairness among these models that are able to fine-tuned by us. We have also clarified the zero setting of the \texttt{GPT-4V} and \texttt{Gemini} models due to their infeasibility to fine-tune them locally.

\vspace{1em}\noindent{\bf \red{Comment 5:} \emph{ALOE and human results are missing from Table 4}} \\
\noindent{\bf \red{Response 5:}} 

Thank you for bringing this to our attention. In response to your comment, we conducted additional experiments during the revision period. Specifically, we evaluated both \textbf{ALOE} and human performance on the real-world data, obtaining results consistent with the simulated dataset trends. We have incorporated these updated results into Table~\ref{tb:real} and Table~{\blue{4}} in the revised manuscript to provide a comprehensive comparison and address this gap clearly.


\vspace{1em}\noindent{\bf \red{Comment 6:} \emph{Design of PCR might overfit to ComPhy. E.g., Physical Property Inferencer has dedicated Mass Graph and Charge Graph to predict object mass and relative charge. It is not feasible to have a dedicated module for every physical property in the world. PCR also has a property-based dynamic predictor to obtain predictions with counterfactual property labels. Counterfactual questions constitute 50\% of all the questions in the dataset. It may give PCR unfair advantages over other baselines.}}

\noindent\textbf{\red{Response 6:}}

\paragraph{Modular Reasoning with Hidden Physical Properties.}
We thank the reviewer for highlighting this concern. While our PCR framework currently employs specialized modules (e.g., Mass Graph and Charge Graph) to infer mass and relative charge properties specifically tailored for the \dataset dataset, the underlying intention is to illustrate the strength of modular reasoning with hidden physical properties, rather than overfitting to particular tasks.

Importantly, PCR's design emphasizes \textbf{modularity} and \textbf{generalizability}. The Physical Property Inferencer (PPI) employs a generalized graph neural network (GNN) structure designed to adapt flexibly to a range of object-centric and relational physical properties. Additional properties can readily be integrated into the existing architecture without significant restructuring. To further demonstrate generalization, in \textbf{Response 3 to Reviewer \#2}, we illustrated how modules trained within PCR could effectively integrate with large vision-language models and image diffusion techniques to solve broader commonsense reasoning tasks, such as object stability (Fig.~\ref{fig:code1}) and video editing scenarios (Fig.~\ref{fig:code2}).

\paragraph{Counterfactual Question Portion.}
Concerning the proportion of counterfactual questions in the dataset, we acknowledge that counterfactual reasoning constitutes a significant portion of the benchmark. However, this choice mirrors the cognitive complexity of physical reasoning tasks frequently encountered by humans. Evaluating hypothetical scenarios through counterfactual reasoning is essential to robust cognitive performance. Therefore, we argue that PCR's dedicated counterfactual reasoning capabilities reflect a core reasoning requirement rather than an unfair advantage. Additionally, PCR consistently outperforms baselines across all question types—not only counterfactual—achieving notably higher accuracy on factual questions (76.0 vs. 68.6) and predictive questions (62.0 vs. 47.1) compared to the best baseline models, as detailed in Table~\blue{3}. Thus, PCR's strong performance across diverse reasoning categories further supports its robustness and general applicability, rather than indicating dataset-specific overfitting.




==> text/response_to_reviewer2_new_v1.tex <==
\textbf{\red{\section{Response to Reviewer \# 2}}}

\vspace{1em}\noindent{\bf \red{Comment 1:} \emph{The ``ComPhy" dataset that was introduced in ICLR 2022 and the one in this manuscript differ in terms of the additional real world videos. However the paper in numerous places states "we introduce a novel benchmark" instead of citing [49] and saying that in the submitted manuscript an extension/update is proposed. I don't think this is appropriate. ICLR papers are archival full conference papers and there shouldn't be an overlap of claims between ICLR and T-PAMI. I would encourage the authors to revise the manuscript to reflect this.}} \\
\noindent\textbf{\red{Response 1:}}

Thank you for highlighting this important issue. We acknowledge that the current manuscript builds upon our previous work presented in ICLR 2022~\cite{chen2021grounding}, and we have accordingly revised the paper to clearly reflect that the \dataset introduced here is an extension and update rather than a completely new benchmark. We have highlighted the revised description in \revise{red} color in the revised paper in different sections. Specifically, we have explicitly cited our prior work~\cite{chen2021grounding} when referring to the dataset and clarified throughout the manuscript that the current submission includes important extensions, such as the inclusion of more diverse physical simulated scenes, real-world videos, and additional analyses. We appreciate your valuable feedback and have made sure to clearly differentiate the contributions and novel extensions presented in this paper relative to our earlier publication. 

\vspace{1em}\noindent{\bf \red{Comment 2:} \emph{The authors should rephrase some of the claims that overlap with the ICLR version.}} \\
\noindent\textbf{\red{Response 2:}} 

Thank you for pointing out this important concern. We have carefully reviewed the manuscript and revised several sentences to clearly differentiate this submission from our previously published ICLR 2022 version~\cite{chen2021grounding}. Specifically, we have rephrased overlapping claims and emphasized the incremental contributions introduced in this paper, including: (1) the addition of more diverse physical simulated scenes, (2) the introduction of a new real-world video dataset for physical reasoning, (3) the development of a new neuro-symbolic model \modelNewFull (\modelNew), and (4) the inclusion of new experiments involving recent large vision-language models (LVLMs). These changes aim to highlight the novel aspects of this submission and ensure transparency regarding the distinctions from our earlier work. We greatly appreciate your suggestion, which helped us improve the clarity and 
positioning of our manuscript. Specifically, we have the following revisions.

\begin{itemize}
    \item \textbf{Introduction Section:}
    \begin{itemize}
        \item Added a citation to the ICLR 2022 version of ComPhy~\cite{chen2021grounding} and clarified that this paper extends the dataset and the method in different ways (~\revise{Line 57-62 and Line 91-95}).
        \item Clearly listed the new contributions over the prior version: a more diverse physical simulated scenes, a new real-world dataset, the proposed \modelNew model, and new LVLM evaluations (~\revise{Line 103-119}). 
    \end{itemize}

    \item \textbf{Related Work Section:}
    \begin{itemize}
        \item Clarified that \dataset is an extension of ComPhy introduced in ICLR 2022~\cite{chen2021grounding}(~\revise{Line 152-153}).
        \item Updated the dataset comparison paragraph to describe \dataset as an extended benchmark rather than an entirely new one (~\revise{Line 185-186}).
    \end{itemize}

    \item \textbf{Dataset Section:}
    \begin{itemize}
        \item In the video generation subsection, it was explained that the pipeline (Bullet + Blender) was reused from the original paper, with new diversity enhancements added (~\revise{Line 248-250}).
        \item In the real-world dataset subsection, explicitly stated that the real-world split is newly introduced in this submission to test real-world transfer (~\revise{Line 353}).
    \end{itemize}
    \item \textbf{Model Section:}
    \begin{itemize}
        \item Added a new discussion describing the simulated scene diversity and clarified that this is a new contribution in this work (~\revise{Line 866-898}).
        \item Added a new discussion describing the real-world scene performance (~\revise{Line 899-908}).
    \end{itemize}
\end{itemize}

\noindent{\bf \red{Comment 3:} \emph{The experiments with SOTA LVLMs are interesting. The draft states "the inferior performance of large vision-language models (LVLMs) is attributed to a gap in their training. These models are pretrained on internet data, which primarily focuses on object categories and semantic relations, lacking emphasis on physical commonsense". I wonder if the proposed method PCR can be integrated with LVLMs like GPT-4V or Gemini and combine the strengths of both approaches? A small discussion on this angle could help.}} 

\noindent{\textbf{\red{Response 3:}}}

Please refer to the \hyperlink{genresp3}{\red{\textbf{Response to General Concern 3}}}. 

\noindent{\bf \red{Comment 4:} \emph{ Adding references related to ComPhy.}} \\
\noindent{\textbf{\red{Response 4:}}}

Thank you for the helpful suggestion. We have revised the Related Work section to include a discussion of CRIPP-VQA~\cite{patel2022cripp}, which presents a benchmark for reasoning about implicit physical properties such as mass and friction through question answering over synthetic videos. While CRIPP-VQA focuses on counterfactual reasoning from individual videos with simple shapes and scenes, our dataset (\dataset) extends these ideas by introducing more diverse and visually complex physical scenes and including real-world videos and by formulating a few-shot setting where models must infer object-centric intrinsic properties from limited interactions across multiple reference videos.
